A Fully Abstract Model of PCF Based on Extended Addressing Machines

Extended addressing machines (EAMs) have been introduced to represent higher-order sequential computations. Previously, we have shown that they are capable of simulating -- via an easy encoding -- the operational semantics of PCF, extended with explicit substitutions. In this paper we prove that the simulation is actually an equivalence: a PCF program terminates in a numeral exactly when the corresponding EAM terminates in the same numeral. It follows that the model of PCF obtained by quotienting typable EAMs by a suitable logical relation is adequate. From a definability result stating that every EAM in the model can be transformed into a PCF program with the same observational behavior, we conclude that the model is fully abstract for PCF.

==> include/old_eam.tex <==
% !TEX root = ../LMCS.tex
%!TEX spellcheck = en-US

We recall the main definitions and properties of \emph{extended addressing machines} (EAMs). For more details and intuition, consult the introductory paper \cite{IntrigilaMM22}.

\subsection{EAMs --- their structure and operational semantics}

We consider fixed a countably infinite set $\Addrs$ of \emph{addresses}. 
We also fix an infinite subset $\Nat \subsetneq \Addrs$, such that $\Addrs-\Nat$ remains infinite.
The elements of $\Nat$ will be the addresses reserved to numerals---we actually identify $\Nat$ with the set of natural numbers.
Let $\Null\notin\Addrs$ be a ``null'' constant representing an uninitialised register. 
\begin{defi}
\bsub
\item 
	An \emph{$\Addrs$-valued tape} $T$ is a finite ordered list of addresses $T = [a_1,\dots,a_n]$ with each $a_i\in\Addrs$, for $1\le i \le n$.  We denote by $\Tapes$ the set of all $\Addrs$-valued tapes.	
\item
	Let $a\in\Addrs$ and $T,T'\in\Tapes$. We denote by $\Cons a {T}$ the tape having $a$ as first element and $T$ as tail. We write $\appT{T}{T'}$ for the concatenation of $T$ and $T'$, which is an $\Addrs$-valued tape.

\item
	Given an index $i \ge 0$, an $\Addrs$-valued \emph{register} $R_i$ is a memory-cell capable of storing either $\Null$ or an address $a\in\Addrs$. We write $\val{R_i}$ to represent the value stored in the register $R_i$. (The notation $\oc R_i$ is borrowed from ML, where $\oc$ represents a dereferencing operator.)
\item
	Given $\Addrs$-valued registers $R_0,\dots,R_r$ for $r\ge 0$, an address $a\in\Addrs$ and an index $i\ge 0$, we write $\vec R\repl{R_i}{a}$ for the list of registers $\vec R$ where the value of $R_i$ has been updated by setting $\val{R_i} = a$.
Notice that, whenever $i > r$, we assume that $\vec R\repl{R_i}{a} = \vec R$ holds.
\esub
\end{defi}

When $\Addrs$ is clear from the context, we omit `$\Addrs$-valued' and simply say registers and tape. 
Besides having registers and tape, each EAM is endowed with a program. Instructions are:
\begin{itemize}
\item $\Load i$ : `pops' the address $a$ from the input tape $\Cons a {T}$ and stores it in the register $R_i$.
If the tape is empty then the machine halts its execution. 
\item $\Apply ijk$ : reads $a_1,a_2$ from $R_i$ and $R_j$ respectively, and stores in $R_k$ the address of the machine obtained by extending the tape of the machine having address $a_1$ with $a_2$. 
\item $\Call i$ : transfers the computation to the machine having as address the value stored in $R_i$, whose tape is extended with the remainder of the current machine's tape.
\item $\Ifz i j k l$: implements the ``\emph{is zero?}'' test on $!R_i$. The instruction needs $\val R_i\in\Nat$.
If $\val R_i = 0$ then the value of $R_j$ is stored in $R_l$, otherwise it is $\val R_k$ that is stored in $R_l$.
\item $\Pred i j$: if $\val{R_i} \in\nat$ then the value of $R_j$ becomes $\val{R_i}\ominus1 := \max\set{\val{R_i} - 1, 0}$.
\item $\Succ i j$: if $\val{R_i} \in\nat$ then the value of $R_j$ becomes $ \val{R_i}+1$.
\end{itemize}

\begin{defi}\label{def:progs}
\bsub
\item \label{def:progs1}
	A \emph{program} $P$ is a finite list of instructions generated by the following grammar, where $\varepsilon$ represents the empty string and $i,j,k,l$ are indices of registers:
	\[
	\begin{array}{lcl}
	\ins{P}&::=&\Load i; \ins{P}\mid \ins{A}\\
	\ins{A}&::=&\Apply ijk; \ins{A}\mid \Ifz ijkl; \ins{A}\mid
	\Pred ij; \ins{A}\mid\Succ ij; \ins{A}\mid\ins{C}\\
	\ins{C}&::=&\Call i \mid \varepsilon
	\end{array}
	\]
	So, a program starts with a list of $\ins{Load}$'s, continues with a list of $\ins{App}$, $\ins{Test}$, $\ins{Pred}$, $\ins{Succ}$, and possibly ends with a $\ins{Call}$. Each of these lists may be empty.
	\item We write $\Load {(i_1, \dots, i_n)}$ as an abbreviation for $\Load{i_1};\,\cdots;\,\Load{i_n}$. 
	\item We write $(\Load {i})^n$ as an abbreviation for a sequence of $\Load i$ of length $n$. 

\item\label{def:progs2}
	We say that a program $P$ is \emph{valid} w.r.t.\ registers $R_0,\dots,R_{r}$, in symbols $\vec R\models P$, if it does not attempt at reading an uninitialized register in $\vec R$ or an $R_j$ for some $j > r$.
\esub
\end{defi}

We allow valid programs to try storing a value $a$ in an unexisting register---as a result the value $a$ will be simply thrown away. We only forbid attempts at reading invalid registers.
The property $\vec R\models P$ is defined precisely in~\cite{IntrigilaMM22}, where it is shown that it is decidable. 

In order to provide some examples, we specify the validity of the following programs w.r.t.\ $R_0 = 7, R_1 = a, R_2 = \Null$.
\[
\bar{lr}
%P_1 = \Pred 02;\Call 2\hfill\textrm{(valid)}\\
P_1 = \Load (2,8);\Ifz 0120; \Call 0&\textrm{(valid: loading $R_2$ before reading it)}\\
P_2 = \Load (0, 2,8); \Call 8&\mathllap{\textrm{(not valid: calling the unexisting register $R_8$)}}\\
P_3 = \Pred 20;\Call 1&\mathllap{\textrm{(not valid: reading the uninitialized register $R_2$)}}
\ear
\]

Hereafter, we will focus on EAMs having valid programs.

\begin{defi}\label{def:AM}
\bsub
\item
	An \emph{extended addressing machine} (\emph{EAM}) $\mM$ over $\Addrs$ (having $r+1$ registers) is given by a tuple $\mM = \tuple{R_0,\dots,R_{r},P,T}$
where 
\begin{itemize}
	\item $\vec R$ are $\Addrs$-valued registers, 
	\item $P$ is a program valid w.r.t.\ $\vec R$, and
	\item $T\in\Tapes$ is an (input) tape.
\end{itemize}
\item We denote by $\cM$ the set of all extended addressing machines over $\Addrs$.
\item
	Given an EAM $\mM$, we write $\mM.\vec R$ for the list of its registers, $\mM.R_i$ for its $i$-th register, $\mM.P$ for the associated program and $\mM.T$ for its input tape.
\item 
	Given $\mM\in\cM$ and $T'\in\Tapes$, we write $\appT{\mM}{T'}$ for the machine 
	\[
	\tuple{\mM.\vec R,\mM.P,\appT{\mM.T}{T'}}.
	\]
\item For $n\in\nat$, the \emph{$n$-th numeral machine} is defined as $\mach{n}= \tuple{R_0,\varepsilon,[]}$, with $\val{R_0} = n$.
\item\label{def:AM6} 
	 For every $a\in\Addrs$, define the following extended addressing machine:
\[
	\mY^a = \tuple{R_0 = \Null,R_1=\Null ,\Load (0, 1);\Apply  0 1 0;\Apply 101; \Call 1,[a]}.
\] 
\esub
\end{defi} 

We now give the details of the addressing mechanism constituting the core of this formalism.

\begin{defi} \label{def:bijectivelookup+Y} Recall that $\nat$ stands for an infinite subset of $\Addrs$ and that $\mY^a$ has been introduced in Definition~\ref{def:AM}(\ref{def:AM6}).
\begin{enumerate}
\item We fix an \emph{address table map} (\emph{ATM}), i.e.\ a bijective function $\Lookup\, :\, \cM \to  \Addrs$ satisfying:
	\begin{enumerate}
	\item (Numerals)
	$\forall n \in \mathbb{N}\,.\, \Lookup{\mach{n}} = n$, where $\mach{n}$ is the $n$-th numeral machine;
\item\label{itemB}
	(Fixed point combinator) $\exists a\in\Addrs-\nnat[]\,.\,\Lookup(\mY^{a}) = a$.
	\end{enumerate}
\item\label{def:ymachine}
	We write $\mY$ for the EAM $\mY^a$ satisfying $\Lookup(\mY^a) = a$ (which exists by \eqref{itemB}).	
\item Given $\mM\in\cM$, we call the element $\Lookup \mM$ the {\em address of the EAM $\mM$}. 
	Conversely, the EAM having as address $a\in\Addrs$ is denoted by $\Lookinv{a}$, i.e.\ $\Lookinv{a} = \mM\iff \Lookup\mM = a.$
\item
	Define the \emph{application map} $(\App{}{}) : \Addrs\times\Addrs\to \Addrs$ by setting 
	\[\App{a}{b} = \Lookup (\append{\Lookinv{a}}{b}).\]
	I.e., the \emph{application} of $a$ to $b$ is the unique address $c$ of the EAM obtained by appending $b$ at the end of the input tape of the EAM $\Lookinv{a}$.	  	
\esub
\end{defi}

The above presentation constitutes a slight improvement over the formulation of \cite{IntrigilaMM22}, where it is assumed the existence of countably many fixed point combinators of different arities.
Such a modification is unessential and does not affect the properties of the system.

\begin{rems}\label{rem:sillyEAMs}
\bsub\item Since $\cM$ and $\Addrs$ are both countable,  the existence of $2^{\aleph_0}$ ATMs follows from cardinality reasons. This includes effective maps as well as non-computable ones.
\item\label{rem:sillyEAMs2} Depending on the chosen address table map, there might exist infinite (static) chains of EAMs, e.g., EAMs  $(\mM_n)_{n\in\nat}$ satisfying
$\mM_n = \tuple{R_0,\varepsilon,[]}$ with $\val R_0 = \Lookup\mM_{n+1}$.
\esub
\end{rems}
The results presented in this particular paper are independent from the choice of the ATM.
\begin{exas}\label{ex:extabsmach} 
The following are examples of EAMs (with uninitialized registers). 
\bsub
\item $\mach{I} := \tuple{R_0, \Load 0; \Call 0, []}$ and $\mach{\appT{Y}{[\Lookup I]}}$ represent the  terms $\comb{I}$ and $\fix(\comb{I})$, respectively.
\item $\mach{Succ1} := \tuple{R_0, \Load 0; \Succ 0 0; \Call 0, []}$. 
Calling $a_{\mach{S}} = \Lookup{\mach{Succ1}}$, one defines:
\item $\mach{Succ2} := \tuple{R_0, R_1, \Load (0,1); \Apply 0 1 1; \Apply 0 1 1; \Call 1,[a_{\mach{S}}]}$.
\esub
\end{exas}
We endow EAMs with a deterministic small-step operational semantics.
%The reduction strategy is deterministic, since the only applicable rule at every step is univocally determined by the first instruction of the internal program, the contents of the registers and the head of the tape.

\begin{defi} \label{def:eamred}
\bsub
\item On EAMs, define a \emph{single-step reduction strategy} as the least relation $\redh\ \subseteq\cM\times\cM$ closed under the rules in Figure~\ref{fig:am:small_step}.
\item The \emph{multistep reduction} $\reddh$ is defined as the transitive-reflexive closure~of~$\redh$.
\item The \emph{conversion relation} $\convh$ is the transitive-reflexive-symmetric closure~of~$\redh$.
\item The \emph{length} of a reduction sequence $\mM\reddh\mN$ is denoted by $\len{\mM\reddh\mN}$.
 \item For $n\ge 0$, we write $\mM\reddh^{n}\mN$ whenever $\mM \reddh \mN$ and $\len{\mM \reddh \mN} = n$ hold.
\esub
\end{defi}
\begin{figure*}[t!]
\centering
{\bf Unconditional rewriting rules}
\[
	\bar{rcl}
	\tuple{\vec R,\Load i;P,\Cons a{T}} &\redh& \tuple{\vec R[R_i := a],P,T}\\
	\tuple{\vec R,\Apply i j k; P,T}&\redh&\tuple{\vec R[R_k := \App{\val{R_i}}{\val{R_j}}],P,T}\\
	\tuple{\vec R,\Call i,T}&\redh&\appT{\Lookinv{\val{R_i}}}{T}\\	
	\ear
\]
{\bf Under the assumption that $\val{R_i} \in \nat$.}
\[
	\bar{rcl}
	\tuple{\vec R,\Pred i j;P,T} &\redh& 
	\tuple{\vec R[R_j := \val{R_i} \ominus 1,P,T},\textrm{ where }n\ominus1 := \max\set{n - 1, 0},\\[1ex]
	\tuple{\vec R,\Succ i j;P,T} &\redh& 
	\tuple{\vec R[R_j := \val{R_i} + 1,P,T}
	\\[1ex]	
	\tuple{\vec R,\Ifz i j k l; P, T}&\redh&\begin{cases}
		\tuple{\vec R[R_l := \val{R_j}], P, T},&\textrm{if }\val{R_i} = 0,\\[3pt]
		\tuple{\vec R[R_l := \val{R_k}], P, T},&\textrm{otherwise}.
		\end{cases}\\
	\ear
\]
{\bf Under the assumption that $\Lookinv{\val{R_i}}\redh \mN$.}
\[
	\bar{rcl}
	\tuple{\vec R,\Pred i j;P,T} &\redh& 
	\tuple{\vec R[R_i := \Lookup{\mN}],\Pred i j;P,T}
	\\
	\tuple{\vec R,\Succ i j;P,T} &\redh& 
	\tuple{\vec R[R_i := \Lookup{\mN}],\Succ i j;P,T}
	\\
	\tuple{\vec R,\Ifz i j k l; P, T}&\redh&\tuple{\vec R[R_i := \Lookup{\mN}],\Ifz i j k l; P, T}\\[-3ex]
	\ear
\]
\caption{Small-step operational semantics for EAMs.}
\label{fig:am:small_step}
\end{figure*}

Given an EAM $\mM$, the first instruction of its program, together with the contents of its registers and tape, univocally determine which rule from Figure~\ref{fig:am:small_step} is applicable (if any).
When $\mM$ tries to perform an arithmetic operation in one of its registers, say $R_i = a$, it needs to wait that the EAM $\Lookinv{a}$ terminates its execution. 
If it does then the success of the operation depends on whether the result is a numeral, otherwise also $\mM$ does not terminate.

\begin{lem}\label{lem:redhproperties}
\bsub\item\label{lem:redhproperties1} 
	The strategy $\redh$ is deterministic: $\mN\,{}_\mach{c}\!\!\leftarrow\mM\redh\! \mN'$ implies $ \mN = \mN'$.
\item\label{lem:redhproperties2} 
	The reduction $\redh$ is Church-Rosser: $\mM\convh\mN \Leftrightarrow \exists \mach{Z}\in\cM\,.\,\mM\reddh \mach{Z} {~}_{\mach{c}}\!\!\twoheadleftarrow\mN$.
\esub
\end{lem}

As a matter of terminology, we say that an EAM $\mM$: 
	\begin{itemize}
	\item is \emph{stuck} %, written $\stuck{\mM}$, 
	if its program has shape $\mM.P = \Load i;P$ but $\mM.T = []$;
	\item \emph{is in an error state} if its program has shape $\mM.P = \ins{ins};P'$ for some instruction $\ins{ins}\in\set{\Load i,\Pred i j,\Succ i j,\Ifz i j k l}$, but $\val{R_i}\notin\nat$ and $\Lookinv{\val{R_i}}\not\redh$.
	\item \emph{is in final state} if $\mM$ is not in an error state, but cannot reduce further, i.e.\ $\mM\not\redh$;
	\item \emph{reaches a final state} (resp.~\emph{raises an error}) if $\mM\reddh\mM'$ for some $\mM'$ in final (resp.\ error) state;  
	$\mM$ \emph{does not terminate}, otherwise.
	\end{itemize}

Consider again the EAMs defined in Example~\ref{ex:extabsmach}.
\begin{exas}  We have (for any $\mM\in\cM$): 
\bsub\item $\appT{\mach{I}}{[\#\mM]} = \tuple{R_0 = \Null, \Load 0; \Call 0, [\Lookup{\mM}]} \redh \tuple{R_0 = \Lookup\mM, \Call 0, []}\redh \mM$; 
\item $\appT{\mach{Y}}{[\#\mach{I}]}\reddh \appT{\mach{I}}{[\#(\appT{\mach{Y}}{[\#\mach{I}]})]}\reddh \appT{\mach{Y}}{[\#\mach{I}]}$; 
\item $\appT{\mach{Succ2}}{[\mach{3}]}\reddh \mach{5}$.
\esub

\end{exas}

\subsection{A type assignment system for EAMs}
\begin{figure*}[t!]
$\bar{ccc}
\infer[(\mathrm{nat})]{\mach{n} : \tint}{}
\qquad
	\infer[(\mathrm{fix})]{\mY{} : (\alpha \to \alpha) \to \alpha}{}&&
	\infer[(\vec R)]{\tuple{R_0,\dots,R_{r},P,T} : \alpha}{R_0,\dots,R_{r} \models \Delta & \Delta\Vdash^r (P,T) : \alpha}
	\\[3pt]
	\infer[(R_\Null)]{R_0,\dots,R_r \models \Delta}{R_0,\dots,R_{r-1} \models \Delta & !R_r = \Null}
	&&
	\infer[(R_\Types)]{R_0,\dots,R_r \models \Delta, r:\alpha}{R_0,\dots,R_{r-1} \models \Delta & \Lookinv{!R_r} : \alpha}
	\\[3pt]
	\infer[(\mathrm{load_{\Null}})]{\Delta \Vdash^r (\Load i;P,[]) : \beta\to\alpha}{\Delta[i : \beta] \Vdash^r (P,[]) : \alpha}
	&&
	\infer[(\mathrm{load_{\Types}})]{\Delta\Vdash^r (\Load i;P, \Cons a {T}) : \alpha}{\Delta[i : \beta] \Vdash^r (P,T) : \alpha & \Lookinv {a} : \beta}
	\\[3pt]
	\infer[(\mathrm{pred})]{\Delta, i : \tint \Vdash^r (\Pred i j;P,T) : \alpha}{(\Delta, i : \tint)[j : \tint] \Vdash^r (P,T) : \alpha}
	&&
	\infer[(\mathrm{succ})]{\Delta, i : \tint \Vdash^r (\Succ i j;P,T) : \alpha}{(\Delta, i : \tint)[j :\tint] \Vdash^r (P,T) : \alpha}
	\\[3pt]
	\multicolumn{3}{c}{\infer[(\mathrm{test})]{\Delta, i : \tint,  j :\beta, k : \beta \Vdash^r (\Ifz i j k l;P,T) : \alpha}{
		(\Delta, i : \tint,  j : \beta, k : \beta)[l : \beta] \Vdash^r (P,T) : \alpha 
		}
	}
	\\[3pt]
	\multicolumn{3}{c}{\infer[(\mathrm{app})]{\Delta, i : \alpha \to \beta, j : \alpha \Vdash^r (\Apply i j k;P,T) : \delta}{
		(\Delta, i : \alpha \to \beta, j : \alpha)[k : \beta] \Vdash^r (P,T) : \delta}	}
	\\[3pt]
	\multicolumn{3}{c}{\infer[(\mathrm{call})]{\Delta, i : \alpha_1\to\dots\to\alpha_n\to\alpha \Vdash^r (\Call i,[\Lookup{\mM_1},\dots,\Lookup{\mM_n}]) : \alpha}{
		 \mM_1 : \alpha_1 & \cdots &  \mM_n : \alpha_n}}
\ear
$
\caption{Typing rules for extended addressing machines.}\label{fig:eamstyping}
\end{figure*}

We introduce a type system for extended addressing machines.

\begin{defi}\label{def:EAMtypes} 
The set $\Types$ of simple types has been introduced in Definition~\ref{def:simpletypes}\eqref{def:simpletypes1}.
\bsub\item A \emph{type environment} is a finite map $\Delta : \nat\to\Types$ represented as a list ${i_1} : \alpha_1,\dots,{i_{n}} : \alpha_{n}$.
Intuitively, $\Delta$ associates (possibly non-consecutive indices of) registers to types.
\item Let $\Delta[i : \alpha]$ be the typing environment $\Delta$ where the type associated with $i$ becomes $\alpha$. 
Note that $\dom(\Delta[i : \alpha]) = \dom(\Delta)\cup\set{i}$. Also, if $i\notin\dom(\Delta)$ then $\Delta[i : \alpha] = \Delta, i : \alpha$.
\item Let $\Delta$ be a typing environment, $\mM\in\cM$, $r\ge 0$, $R_0,\dots,R_r$ be registers, $P$ be a program, $T\in\Tapes$ and $\alpha\in\Types$. We define the typing judgements
\[
	\mM : \alpha\qquad\qquad\qquad	\Delta \Vdash^r (P,T) : \alpha
	\qquad\qquad\qquad R_0,\dots,R_r\models \Delta
\] 
by mutual induction as the least relations closed under the rules of Figure~\ref{fig:eamstyping}.
\item A machine $\mM$ is called \emph{typable} if the judgement $\mM : \alpha$ is derivable for some $\alpha\in\Types$.
\esub
\end{defi}

To type an EAM $\mM$ with $r+1$ registers $\alpha$, one needs to construct a derivation of $\mM : \alpha$. The machines $\mach{n}$ and $\mY$ are recognizable from their addresses and treated as constants. 
Otherwise, the rule $(\vec R)$ checks that the values in the initialized registers $R_{i_1},\dots,R_{i_n}$ are typable $\mM.\vec R \models \Delta$ and retain only their types in $\Delta = {i_1}:\beta_{i_1},\dots,{i_n}:\beta_{i_n}$.
Subsequently, one needs to derive a judgement of the form $\Delta\Vdash^r (\mM.P,\mM.T) : \alpha$ by verifying the coherence of the instructions in the program with the types of the registers and the values in the tape.
The superscript $r\ge 0$ in $\Vdash^r$ keeps track of the initial amount of registers, i.e.\ $\vec i \in\set{0,\dots,r}$.

\begin{prop}[{Intrigila et al.~\cite[Prop.~3.5]{IntrigilaMM22}}]\label{prop:typing} ~\\
Let $\mM,\mN\in\cM$ and $\alpha,\beta\in\Types$.
\bsub
\item\label{prop:typing1}
	If $ \mM : \beta \to \alpha$ and $\mN : \beta$ then $\appT{\mM}{[\Lookup{\mN}]} : \alpha$.
\item\label{prop:typing2}
	If $ \mM : \alpha$ and $\mM\redh \mN$ then $ \mN : \alpha$.
\item\label{prop:typing4}
	If $ \mM : \tint$ then either $\mM$ does not terminate or $\mM\reddh \mach{n}$, for some $n\ge 0$.
\item\label{prop:typing3}
	If $ \mM : \alpha$ then $\mM$ does not raise an error.
\esub
\end{prop}

\begin{exas} The following EAMs have been introduced in Example~\ref{ex:extabsmach}.
\bsub\item
$ \mach{I} : \alpha\to\alpha$, for all $\alpha\in\Types$. In particular $\mach{I} : \tint\to\tint$, whence $\mach{\appT{Y}{[\Lookup I]}} : \tint$.
\item $\mach{Succ1} :\tint\to\tint$ and $\mach{Succ2} : \tint\to\tint$.
\esub
\end{exas}


%\begin{notation}
%Given $\vdash \Lookinv {a_i} : \alpha_i,\dots, \vdash \Lookinv {a_i} : \alpha_j$, $n \in \nat^{+}, n > j$, let $\vec R^n_{a_i,\dots,a_j} = R_0,\dots,R_{n-1}$ such that for all $k < n$, $!R_k \neq \emptyset$ if and only if there exists $a_k \in a_i,\dots,a_j$ and $!R_k = a_k$. 
%\end{notation}
